Room-temperature ladder-type optical memory compatible with single photons from InGaAs quantum dots

On-demand storage and retrieval of quantum information in coherent light-matter interfaces is a key requirement for future quantum networking and quantum communication applications. Alkali vapor memories offer scalable and robust high-bandwidth storage at high repetition rates which makes them a natural fit to interface with solid-state single-photon sources. Here, we experimentally realize a room-temperature ladder-type atomic vapor memory that operates on the Cs D1 line. We provide a detailed experimental characterization and demonstration of on-demand storage and retrieval of weak coherent laser pulses with 0.06 photons per pulse at a high signal-to-noise ratio of SNR$=830(80)$. The memory achieves a maximum internal storage efficiency of $\eta_{\text{int}}=15(1)\%$ and an estimated $1/e$-storage time of $\tau_{\mathrm{s}}\approx32\,$ns. Benchmark properties for the storage of single photons from inhomogeneously broadened state-of-the-art solid-state emitters are estimated from the performance of the memory. Together with the immediate availability of high-quality InGaAs quantum dots emitting at 895\,nm, these results provide clear prospects for the development of a heterogeneous on-demand quantum light interface.

==> backup.tex <==
%The exponential decay accounts for spinwave dephasing due to ballistic motion of the atoms during the storage process. %This motional dephasing is proportional to the length of the spinwave and inversely proportional to the wavevector %mismatch of signal and control laser. The inset of Fig.\,\ref{fig:storagetimescan} depicts this relation. However, it %has been shown that additional off-resonant dressing fields can reduce the residual Doppler broadening and thereby %increase the lifetime of the memory \cite{Davidson:2023}. The Gaussian decay of the spinwave stems from inhomogeneous %decay mechanisms such as spin-exchange collisions, atoms leaving the interaction area, etc. Note that the zero-time %storage efficiency cannot be faithfully determined from the fit. All following data has been acquired at the maximum %efficiency retrieval time of 17.4\,ns.

In Fig.\,\ref{fig:temperature_detail} we show the influence of the temperature on the read-in and read-out efficiencies. We define the read-in efficiency as $\eta_{\text{in}}=1-N_{\text{leak}}/N_{\text{in}}$ where $N_{\text{leak}}$ are the leakage counts. The read-out efficiency is given by  $\eta_{\text{out}}=N_{\text{ret}}/(N_{\text{in}}-N_{\text{leak}})$ such that $\eta_{\text{int}}=\eta_{\text{in}}\cdot\eta_{\text{out}}$. As expected, the absorptive loss $N_{\text{loss}}=1-N_{\text{leak}} - N_{\text{ret}}$ increases with higher temperatures. However, it is not immediately clear why the read-out efficiency has a maximum at $57^\circ$C and decreases for higher temperatures. For the highest temperatures we observe features of partial read-out in the storage traces.  
\begin{figure}[h]%H
\includegraphics[width=\columnwidth]{Figures/temperature_details.png}
\caption{\label{fig:temperature_detail}
Storage and retrieval efficiencies for different temperatures. Repeated storage experiment at 300\,MHz detuning at 17.4\,ns retrieval time for different temperatures of the atomic ensemble. Uncertainties represent fit errors and the accuracy of our heating system.}
\end{figure}


\appendix
\section{Methods}
\label{sec:methods}

\subsection{Spectral acceptance window}
\label{subsec:app_acceptancewindow}

 The data in \ref{fig:bandwidth} can be used to emulate the influence of spectral drifts of the memory input light source during one experiment. The measured data $\mathcal{D} (\Delta,\delta)$ is a convolution of the spectral shape of our input laser $\mathcal{E}(\Delta,\delta)$ and some unknown spectral memory acceptance window $\mathcal{M}(\delta)$ where $\Delta$ is the laser detuning from the atomic transition and $\delta$ is the two-photon detuning from the memory state. For one initial detuning, we can infer the memory acceptance window by deconvolution:
\begin{equation}
\mathcal{D} (\Delta,\delta) = \mathcal{E}(\Delta,\delta) \star \mathcal{M}(\Delta,\delta)
\end{equation}

By virtue of the convolution theorem we can write the memory acceptance window as:

\begin{equation}
\mathcal{M}(\Delta,\delta) = \mathcal{F}^{-1} \left[\frac{\mathcal{F}(\mathcal{D})}{\sqrt{2\pi}\mathcal{F}(\mathcal{E})}\right]
\end{equation}

The result of these calculations can be found in fig.\ref{fig:bandwidth}. From the memory acceptance window we can estimate the expected internal memory efficiency $\eta_{exp}$ for signals $\mathcal{S}$ with different spectral shapes. Under the assumption that the signal is centered in the middle of the acceptance window we can write:

\begin{equation}
    \eta_{exp} (\Delta) = \int_{-\infty}^\infty \text{d} \delta \ \mathcal{M}(\Delta,\delta) \mathcal{S} (\Delta,\delta)
\end{equation}

These results can be used to test the memory on compatibility with various different sources of single photons such as semiconductor quantum dots or cavity enhanced SPDC.

\subsection{Storage time}
\label{subsec:app_storagetime}

The model for the fit of the storage time plot in fig. \ref{fig:storagetimescan} is taken from \cite{Finkelstein:2018}. They assume a beating of the spinwave due to multiple addressed hyperfine states in the 6D$_3/2$ storage state. The envelope is a mixture of an exponential homogeneous decay of the storage state and a Gaussian-shapeed decay from inhomogeneous mechanisms such as residual Doppler-broadening and time-of-flight loss from the interaction area. They provide the following formula:


\begin{eqnarray}
    \eta(t)& = &\eta_0\exp^{-[\frac{1}{\tau_s\bar\tau}(t-t_0-\tau_s)(t-t_0+\bar\tau)+1]}\\
    &&\left| \frac{1+Ae^{-i\omega_{23}(t-t_0)}+Be^{-i\omega_{34}(t-t_0)}+Ce^{-i\omega_{45}(t-t_0)}+De^{-i(\omega_{23}+\omega_{34})(t-t_0)}}{1+A+B+C+D} \right|^2
\end{eqnarray}

where $\omega_{23}$, $\omega_{34}$ and $\omega_{45}$ are the hyperfine splittings of the 6D$_{3/2}$ state. The different decay mechanisms are encoded in the ...

We summarize the fit parameters in the following table:

\begin{table}[b]
\begin{ruledtabular}
\begin{tabular}{cccccccc}
$\eta_0$&$\tau_s$ [ns]&$\bar\tau$ [ns]&$t_0$ [ns]&A&B&C&D\\
\hline
0.71&24.4&24.4&-0.02&1.14&2.79&-0.12&1.45
\end{tabular}
\end{ruledtabular}
\caption{\label{tab:table4}%
Fit parameters used in fig. \ref{fig:storagetimescan}}
\end{table}
